CensorSpoofer: Asymmetric Communication with IP Spoofing for Censorship-Resistant Web Browsing

A key challenge in censorship-resistant web browsing is being able to direct legitimate users to redirection proxies while preventing censors, posing as insiders, from discovering their addresses and blocking them. We propose a new framework for censorship-resistant web browsing called {\it CensorSpoofer} that addresses this challenge by exploiting the asymmetric nature of web browsing traffic and making use of IP spoofing. CensorSpoofer de-couples the upstream and downstream channels, using a low-bandwidth indirect channel for delivering outbound requests (URLs) and a high-bandwidth direct channel for downloading web content. The upstream channel hides the request contents using steganographic encoding within email or instant messages, whereas the downstream channel uses IP address spoofing so that the real address of the proxies is not revealed either to legitimate users or censors. We built a proof-of-concept prototype that uses encrypted VoIP for this downstream channel and demonstrated the feasibility of using the CensorSpoofer framework in a realistic environment.

==> sip.tex <==

\subsection{Background of SIP-based VoIP}
\label{ssec:sip}

VoIP is an Internet service that transmits Voice over IP-based networks. It employs session control protocols, such as SIP, MGCP, and H.323, to setup and tear down calls. SIP is one of the most widely-used VoIP signal protocols, because of its light weight. In this work, we focus on SIP-based VoIP systems.


SIP is an application layer protocol. It can run on either UDP or TCP. There are three main elements in SIP systems: user agents, location services, and servers. 

\begin{itemize}

\item {\it User agents} are the end devices in a SIP network. They originate SIP requests to establish media session, and send and receive media. A user agent can be a physical SIP phone or SIP client software running on a computer (also called {\it softphone}). A user agent needs a SIP ID, which is signed up at a SIP provider, in order to make and receive SIP calls.

\item {\it Location service}  is a database that contains information about users, such as SIP IDs, the latest login IP addresses, preferences, etc. Location services generally do not interact directly with user agents. 

\item {\it Servers} are intermediary devices that are located within the SIP network and assist user agents in session establishment. There are two main types of SIP servers: {\it registrar} and {\it proxy}.  A registrar receives SIP registration requests and updates the user agent's information (such as the login IP address) into the location service. A SIP proxy receives SIP requests from a user agent or another proxy and forwards the request to another location.

\end{itemize}

%\subsubsection{SIP Session Setup} 

Here is an example to show how a user (Alice) calls another user (Bob). Suppose Alice has signed up a SIP ID \texttt{alice@atlanta.com} at the SIP provider \texttt{atlanta.com}, and Bob got his SIP ID \texttt{bob@biloxi.com} from \texttt{biloxi.com}, and  Alice knows Bob's SIP ID.

When Bob comes online, he first sends a registration request to the registrar of \texttt{biloxi.com} with its current IP address. 
So does Alice to register herself at the registrar of \texttt{atlanta.com}.

\begin{figure}[t]
	\centering
	\includegraphics[width=8cm]{sip_v2.eps}
	\caption{An example of a SIP session (registrars and location services are not shown).}
	\label{fig:sip}
\end{figure}

The SIP call initialization process is shown in Figure~\ref{fig:sip}. First, Alice sends an INVITE message (M1), which contains her SIP ID and IP address, Bob's SIP ID, her supported media codecs, etc., to the proxy of \texttt{atlanta.com} (note that  at this point Alice does not know Bob's IP address). The local proxy performs a DNS lookup to find the IP address of the proxy serving Bob's domain, i.e., \texttt{biloxi.com}, and then forwards the INVITE message (M2) to the remote proxy. At the meantime, the local proxy sends a Trying response (M3) back to Alice, indicating that the INVITE has been received and is being routed to the destination. Upon receiving the INVITE message, the proxy of \texttt{biloxi.com} sends a query to its location service to look up the registered IP address of Bob, and then it forwards the INVITE message (M4) to Bob. The user agent of Bob sends a Ringing response (M6) to the proxy indicating that Bob's phone is ringed. If Bob decides to answer the phone, an OK message containing Bob's current IP (M9) is sent and forwarded back to Alice; otherwise, a Reject response is returned (not shown in the figure). From the received OK message, Alice learns Bob's IP address, and sends an ACK message towards Bob (M12, M13, M14). At this point, the SIP initialization session is done, and Alice and Bob start the media session by sending each other audio data directly. At the end of the media session, either party can send a BYE message (M15) to close the call.


The media session uses Real-time Transport Protocol (RTP) to transmit audio data, and Real-time Transport Control Protocol (RTCP) to provide out-of-band statistic and control information for the RTP flow. Both RTP and RTCP run on top of UDP. 
VoIP clients can use SRTP/SRTCP~\cite{srtp}---an encrypted version of RTP/RTCP---to encrypt their voice communication. SRTP/SRTCP only requires the user to install a user agent that supports RTP/RTCP encryption, and does not require the VoIP servers to support encryption. This implies that the user can use any VoIP provider, including local providers that collude with the censor, to access our circumvention system. Currently, there are many VoIP clients supporting SRTP and/or ZRTP, such as Blink~\cite{blink}, SFLphone~\cite{sflphone}, Zfone~\cite{zfone}, and PJSUA~\cite{pjsua}. The encryption key for SRTP/SRTCP can be either established beforehand, e.g., via MIKEY~\cite{mikey}, or negotiated on the fly using ZRTP~\cite{zrtp}. In this work, we consider using pre-established keys for SRTP/SRTCP.

